Balance Transfers and Bailouts in Credit Networks using Blockchains

In this paper, we propose a technique for rebalancing link weights in decentralized credit networks. Credit networks are peer-to-peer trust-based networks that enable fast and inexpensive cross-currency transactions compared to traditional bank wire transfers, which has led to their increasing popularity and use. Although researchers have studied security of transactions and privacy of users of such networks, and have invested significant efforts into designing efficient routing algorithms for credit networks, comparatively little work has been done in the area of {replenishing} credit links of users in the network. Replenishing links at regular intervals in a credit network is important to keep users solvent, the network viable with enough liquidity, and to prevent transaction failures. This is achieved by a process called {rebalancing} that enables a poorly funded user to create incoming as well as outgoing credit links. We propose a system where a user with zero or no link weights can create incoming links with existing, trusted users in the network, in a procedure we call {balance transfer}, followed by creating outgoing links to existing or new users that would like to join the network, a process we call {bailout}. Both these processes together constitute our proposed rebalancing mechanism. Our techniques would also serve to make the network more competitive by offering users lower rates of interest, and enable users to earn routing fees-based revenue by participating in high throughput transaction paths.

==> Discussion.tex <==
\section{Discussion}
\label{sec:disc}

In this section, we discuss the possible outcomes and constraints of the proposed balance transfer and bailout design. 
In the balance transfer algorithms, we use the two different routing schemes, prefix embedding and Chord. When we use Chord routing algorithm, we notice that this would provide an limitation on number of users in the network. This kind of routing can also be done using other similar routing techniques such as pastry or Tapestry. In both of these routing algorithms, we involve an arbitrator to find any malicious activity between colluding users. Such an arbitrator can find the part of the path where a packet or response has been dropped/forwarded to a wrong user, but cannot exactly point to the user causing malicious activity. This can be further mitigated by improving the routing mechanism. Further, in the bailout mechanism, we introduce landmark nodes to assist the users in establishing outgoing link. It is important to note that, the landmark nodes are not used for any payment across the network which enables us to retain the properties of credit network, also reducing the trust placed in such landmark nodes.

 
